SGIFormer: Semantic-guided and Geometric-enhanced Interleaving Transformer for 3D Instance Segmentation

In recent years, transformer-based models have exhibited considerable potential in point cloud instance segmentation. Despite the promising performance achieved by existing methods, they encounter challenges such as instance query initialization problems and excessive reliance on stacked layers, rendering them incompatible with large-scale 3D scenes. This paper introduces a novel method, named SGIFormer, for 3D instance segmentation, which is composed of the Semantic-guided Mix Query (SMQ) initialization and the Geometric-enhanced Interleaving Transformer (GIT) decoder. Specifically, the principle of our SMQ initialization scheme is to leverage the predicted voxel-wise semantic information to implicitly generate the scene-aware query, yielding adequate scene prior and compensating for the learnable query set. Subsequently, we feed the formed overall query into our GIT decoder to alternately refine instance query and global scene features for further capturing fine-grained information and reducing complex design intricacies simultaneously. To emphasize geometric property, we consider bias estimation as an auxiliary task and progressively integrate shifted point coordinates embedding to reinforce instance localization. SGIFormer attains state-of-the-art performance on ScanNet V2, ScanNet200 datasets, and the challenging high-fidelity ScanNet++ benchmark, striking a balance between accuracy and efficiency. The code, weights, and demo videos are publicly available at https://rayyoh.github.io/sgiformer.

==> sections/6_limitations.tex <==
\section{Limitations and Future Work}\label{sec:limitations}

==> table/ablation_decoder.tex <==
\begin{tabular}{x{10mm}x{10mm}x{10mm}|x{10mm}x{10mm}x{10mm}}
    \toprule
    \smq & \geid & Vanilla & mAP &AP$_{50}$ & AP$_{25}$ \\
    \midrule
    \YesV &  & \YesV & 57.9 & 77.6 & 85.6 \\
    \cellcolor[HTML]{efefef}\YesV & \cellcolor[HTML]{efefef}\YesV & \cellcolor[HTML]{efefef} & \cellcolor[HTML]{efefef}58.9 & \cellcolor[HTML]{efefef}78.4 & \cellcolor[HTML]{efefef}86.2 \\
    \bottomrule
\end{tabular}

==> table/efficiency.tex <==
\begin{tabular}{x{22mm}|x{15mm}x{15mm}x{15mm}}
    \toprule
    Methods & Params.(M)$\downarrow$ & FLOPs(G)$\downarrow$ & Latency(ms)$\downarrow$ \\
    \midrule
    SoftGroup \cite{vu2022softgroup} & 30.84 & x & x \\
    Mask3D \cite{schult2023mask3d} & 39.62 &  x & x \\
    SPFormer \cite{sun2023spformer} & 17.60 & x & x \\
    OneFormer3D \cite{kolodiazhnyi2023of3d} & 17.52 & x & x \\
    Sph. Mask \cite{shin2023spherical} & 30.77 & x & x \\
    % ISBNet \cite{ngo2023isbnet} & 30.72 &54.4 &73.1 &82.5 \\
    \midrule
    Ours-Tiny & 15.96 & x & x \\
    Ours & 35.11 & x & x \\
    \bottomrule
\end{tabular}
